Natural continual learning: success is a journey, not (just) a destination

Biological agents are known to learn many different tasks over the course of their lives, and to be able to revisit previous tasks and behaviors with little to no loss in performance. In contrast, artificial agents are prone to 'catastrophic forgetting' whereby performance on previous tasks deteriorates rapidly as new ones are acquired. This shortcoming has recently been addressed using methods that encourage parameters to stay close to those used for previous tasks. This can be done by (i) using specific parameter regularizers that map out suitable destinations in parameter space, or (ii) guiding the optimization journey by projecting gradients into subspaces that do not interfere with previous tasks. However, these methods often exhibit subpar performance in both feedforward and recurrent neural networks, with recurrent networks being of interest to the study of neural dynamics supporting biological continual learning. In this work, we propose Natural Continual Learning (NCL), a new method that unifies weight regularization and projected gradient descent. NCL uses Bayesian weight regularization to encourage good performance on all tasks at convergence and combines this with gradient projection using the prior precision, which prevents catastrophic forgetting during optimization. Our method outperforms both standard weight regularization techniques and projection based approaches when applied to continual learning problems in feedforward and recurrent networks. Finally, the trained networks evolve task-specific dynamics that are strongly preserved as new tasks are learned, similar to experimental findings in biological circuits.

==> __latexindent_temp.tex <==
\section{Method}
\label{sec:method}

\paragraph{Notations} We use  $\b{X}^\top$, $\b{X}^{-1}$, $\text{Tr}(\b{X})$ and $\text{vec}(\b{X})$ to denote the transpose, inverse, trace, and column-wise vectorization of a matrix $\b{X}$.
We use $\b{X} \otimes \b{Y}$ to represent the Kronecker product between matrices $\b{X} \in \mathbb{R}^{n \times n}$ and $\b{Y} \in \mathbb{R}^{m \times m}$ such that $(\b{X} \otimes \b{Y})_{mi + k ,m j + l }  = \b{X}_{ij} \b{Y}_{kl}$.
We use bold lower-case letters $\b{x}$ to denote column vectors.
$\mathcal{D}_k$ refers to a `dataset' corresponding to task $k$, which in this work generally consists of a set of input-output pairs $\{ \b{x}_k^{(i)}, \b{y}_k^{(i)} \}$ such that $\ell_k(\b{\theta}) := \log p(\mathcal{D}_k | \b{\theta}) = \sum_i \log p_{\b\theta}(\b{y}^{(i)}_k | \b{x}^{(i)}_k)$ is the task-related performance on task $k$ for a model with parameters $\b{\theta}$.
Finally, we use $\hat{\mathcal{D}}_k$ to refer to a dataset generated by inputs from the $k^{th}$ task where $ \{ \hat{\b{y}}_k^{(i)} \sim p_{\b\theta}(\b{y} | \b{x}^{(i)}_k) \}$ are drawn from the model distribution $\mathcal{M}$.

\subsection{Bayesian continual learning}
\label{subsec:bcl}

\paragraph{Problem statement}
In continual learning, we train a model on a set of $K$ tasks $\{ \mathcal{D}_1, \ldots, \mathcal{D}_K \}$ that arrive sequentially, where the data distribution $\mathcal{D}_k$ for task $k$ in general differs from $\mathcal{D}_{\neq k}$.
The aim is to learn a probabilistic model $p(\mathcal{D}|\b{\theta})$ that performs well on all tasks.
The challenge in the continual learning setting stems from the sequential nature of learning, and in particular from the common assumption that the learner does not have access to ``past'' tasks (i.e., $\mathcal{D}_j$ for $j < k$) when learning task $k$.
While we enforce this stringent condition in this paper, our approach may be easily combined with memory-based techniques such as coresets or generative replay \citep{ehret2020continual,von2019continual,nguyen2017variational,pan2020continual,shin2017continual,van2020brain,cong2020gan,rebuffi2017icarl,de2020continual,rolnick2019experience,titsias2020functional}.


\paragraph{Bayesian approach}
The continual learning problem is naturally formalized in a Bayesian framework whereby the posterior after $k-1$ tasks is used as a prior for task $k$.
More specifically, we choose a prior $p(\b{\theta})$ on the model parameters and compute the posterior after observing $k$ tasks according to Bayes' rule:
%
\begin{align}
	p(\b{\theta} | \mathcal{D}_{1:k}) \nonumber
	 & \propto p(\b{\theta}) \prod_{k'=1}^k p(\mathcal{D}_{k'}|\b{\theta})                         \\
	 & \propto p(\b{\theta}| \mathcal{D}_{1:k-1})  p(\mathcal{D}_k|\b{\theta}), \label{eq:cl_post}
\end{align}
%
where $\mathcal{D}_{1:k}$ is a concatenation of  the first $k$ tasks $(\mathcal{D}_1, \ldots, \mathcal{D}_k)$.
In theory, it is thus possible to compute the exact posterior $p(\b{\theta}|\mathcal{D}_{1:k})$ after $k$ tasks, while only observing $\mathcal{D}_k$, by using the posterior $p(\b{\theta}|\mathcal{D}_{1:k-1})$ after $k-1$ tasks as a prior.
However, as is often the case in Bayesian inference, the difficulty here is that the posterior is typically intractable.
To address this challenge, it is common to perform approximate online Bayesian inference.
That is, the posterior $p(\b{\theta}|\mathcal{D}_{1:k-1})$ is approximated by a parametric distribution with parameters $\b{\phi}_{k-1}$.
The approximate posterior $q(\b{\theta}; \b{\phi}_{k-1})$ is then used as a prior for task $k$.

\paragraph{Online Laplace approximation}
A common approach is to use the Laplace approximation whereby the posterior $p(\b{\theta}|\mathcal{D}_{1:k-1})$ is approximated as a multivariate Gaussian $q$ using local gradient information \citep{kirkpatrick2017overcoming,ritter2018online,huszar2017quadratic}.
This involves (i) finding a mode $\b{\mu}_{k}$ of the posterior during task $k$, and (ii) performing a second-order Taylor expansion around $\b{\mu}_k$ to construct an approximate Gaussian posterior
%
$q(\b{\theta}; \b{\phi}_{k}) = \mathcal{N}(\b{\theta}; \b{\mu}_{k}, \b{\Lambda}_k^{-1})$,
%
where $\b{\Lambda}_k$ is the precision matrix and $\b{\phi}_k = (\b{\mu}_k, \b{\Lambda}_k)$.
%
In this case, gradient-based optimization is used to find the posterior mode on task $k$ (c.f. \Cref{eq:cl_post}):
%
\begin{align}
	\b{\mu}_k
	 & = \argmax_{\b{\theta}}~
	\log p(\b{\theta}|\mathcal{D}_k, \b{\phi}_{k-1})         \\
	 & = \argmax_{\b{\theta}}~
	\log p(\mathcal{D}_k | \b{\theta}) +
	\log q(\b{\theta};\b{\phi}_{k-1})
	\\
	 & = \argmax_{\b{\theta}}~ \underbrace{\ell_k(\b\theta)-
		\frac{1}{2} (\b{\theta} - \b{\mu}_{k-1})^{\top}\b{\Lambda}_{k-1}(\b{\theta} - \b{\mu}_{k-1})}_{\displaystyle := \mathcal{L}_k(\b\theta)}
	\label{eq:laplace_update_mu}
\end{align}
The precision matrix $\b{\Lambda}_k$ is given by the Hessian of the negative log posterior at $\b{\mu}_k$:
%
\begin{align}
	\b{\Lambda}_k
	=
	-\left .
	\nabla_{\b{\theta}}^2 \log p(\b{\theta}|\mathcal{D}_k, \b{\phi}_{k-1})
	\right |_{\b{\theta} = \b{\mu}_k}
	=
	H(\mathcal{D}_k, \b{\mu}_k)
	+
	\b{\Lambda}_{k-1},
	\label{eq:laplace_update_lambda}
\end{align}
%
where $H(\mathcal{D}_k, \b{\mu}_k) =
	-
	\left .
	\nabla_{\b{\theta}}^2 \log p(\mathcal{D}_k | \b{\theta})
	\right |_{\b{\theta} = \b{\mu}_k}$ is the Hessian of the negative log likelihood of $\mathcal{D}_k$.

Continual learning with the online Laplace approximation thus involves two steps for each new task $\mathcal{D}_k$.
First, given $\mathcal{D}_k$ and the previous posterior $q(\b{\theta};\b{\mu}_{k-1}, \b{\Lambda}_{k-1}^{-1})$ (i.e. the new prior), $\b{\mu}_{k}$ is found using gradient-based optimization (\Cref{eq:laplace_update_mu}).
This step can be interpreted as optimizing the likelihood of $\mathcal{D}_k$ while penalizing changes in the parameters $\b{\theta}$ according to their importance for previous tasks, as determined by the prior precision matrix $\b{\Lambda}_{k-1}$.
Second, the new posterior precision matrix $\b{\Lambda}_k$ is computed according to \Cref{eq:laplace_update_lambda}.

\paragraph{Approximating the Hessian}
In practice, computing $\b{\Lambda}_k$ presents two major difficulties.
First, because $q(\b{\theta} ; \b{\phi}_k)$ is a Gaussian distribution, $\b{\Lambda}_k$ has to be positive semi-definite (PSD), which is not guaranteed for the Hessian $H(\mathcal{D}_k, \b{\mu}_k)$.
Second, if the number of model parameters $n_\theta$ is large, it may be prohibitive to compute a full $( n_\theta \times n_\theta)$ matrix.
To address the first issue, it is common to approximate the Hessian with the Fisher information matrix (FIM; \citealp{martens2014new,huszar2017quadratic,ritter2018online}):
%
\begin{align}
	\b{F}_k =
	\left .
	\mathbb{E}_{p(\hat{\mathcal{D}}_k|\b{\theta})}
	\left [
		\nabla_{\b{\theta}} \log p(\hat{\mathcal{D}}_k|\b{\theta})
		\nabla_{\b{\theta}} \log p(\hat{\mathcal{D}}_k|\b{\theta})^{\top}
		\right ]
	\right |_{\b{\theta}=\b{\mu}_k}
	\approx H(\mathcal{D}_k, \b{\mu}_k)
	\label{eq:fisher_k}
\end{align}
%
The FIM is PSD, which ensures that $\b{\Lambda}_k = \sum_{k'=1}^k \b{F}_{k'}$ is also PSD.
Computing $\b{F}_k$ may still be impractical if there are many model parameters, and it is therefore common to further approximate the FIM using structured approximations with fewer parameters.
In particular, a diagonal approximation to $\b{F}_k$ recovers Elastic Weight Consolidation (EWC; \citealp{kirkpatrick2017overcoming}), while a Kronecker-factored approximation~\citep{martens2015optimizing} recovers the method proposed by \citet{ritter2018online}.
We denote this method `KFAC' and use it in \Cref{sec:exps} as a comparison for our own Kronecker-factored method.

\subsection{Natural continual learning}
\label{subsec:ngcl}

\input{figures/_fig_schematic.tex}

While the online Laplace approximation has been applied successfully in several continual learning settings \citep{kirkpatrick2017overcoming,ritter2018online}, it has also been found to perform sub-optimally on a range of problems \citep{van2018generative,duncker2020organizing}.
Additionally, its Bayesian interpretation in theory prescribes a unique way of weighting the contributions of previous and current tasks to the loss.
However, to perform well in practice, weight regularization approaches have been found to require ad-hoc re-weighting of the prior term by several orders of magnitude \citep{kirkpatrick2017overcoming,ritter2018online,van2018generative}.
These shortcomings could be due to an inadequacy of the approximations used to construct the posterior (\Cref{subsec:bcl}).
However, we show in \Cref{fig:schematic} that standard gradient descent on the Laplace posterior has important drawbacks even in the exact case.
First, we show that exact Bayesian inference on a simple continual regression problem can produce indirect optimization paths along which previous tasks are transiently forgotten as a new task is being learned (\Cref{fig:schematic}A; green).
Second, when the loss is non-convex, we show that exact Bayesian inference can still lead to catastrophic forgetting (\Cref{fig:schematic}B; green).

An alternative approach that has found recent success in a continual learning setting involves projection based methods which restrict parameter updates to a subspace that does not interfere with previous tasks \citep{zeng2019continual,duncker2020organizing}.
However, it is not immediately obvious how this projected subspace should be selected in a way that appropriately balances learning on previous and current tasks.
Additionally, such projection-based algorithms have fixed points that are minima of the current task, but not necessarily minima of the (negative) Bayesian posterior.
This can lead to catastrophic forgetting in the limit of long training times (\Cref{fig:schematic}; pink), unless the learning rate is exactly zero in directions that interfere with previous tasks.

To combine the desirable features of both classes of methods, we introduce ``Natural Continual Learning'' (NCL) -- an extension of the online Laplace approximation that also restricts parameter updates to directions which do not interfere strongly with previous tasks.
In a Bayesian setting, we can conveniently express what is meant by such directions in terms of the prior precision matrix $\b{\Lambda}$.
In particular, `flat' directions of the prior (low precision) correspond to directions that will not significantly affect the performance on previous tasks.
Formally, we derive NCL as the solution of a trust region optimization problem.
This involves minimizing the posterior loss $\mathcal{L}_k(\b{\theta})$ within a region of radius $r$ centered around $\b{\theta}$ with a distance metric of the form $d(\b{\theta}, \b{\theta}+\b{\delta}) = \sqrt{\b{\delta}^\top \b{\Lambda}_{k-1} \b{\delta} /2}$ that takes into account the curvature of the prior via its precision matrix $\b{\Lambda}_{k-1}$:
%
\begin{align}
	 & \b{\delta}
	=
	\argmin_{\b{\delta}}
	\mathcal{L}_k(\b{\theta})
	+
	\nabla_{\b{\theta}} \mathcal{L}_k(\b{\theta})^\top
	\b{\delta}
	\quad
	\text{subject to}
	\;\;
	\frac{1}{2}\b{\delta}^\top \b{\Lambda}_{k-1} \b{\delta} \leq r^2,
	\label{eq:ncl_trust_region}
\end{align}
%
where
$
	\mathcal{L}_k(\b{\theta} + \b{\delta}) \approx
	\mathcal{L}_k(\b{\theta}) +
	\nabla_{\b{\theta}} \mathcal{L}_k(\b{\theta})^\top \b{\delta}$
is a first-order approximation to the updated Laplace objective.
The solution to this subproblem is given by
$\b{\delta} \propto \b{\Lambda}_{k-1}^{-1} \nabla_{\b{\theta}} \ell_k(\b{\theta}) - (\b{\theta} - \b{\mu}_{k-1})$ (see \CrefNoLink{sec:alt_ncl} for a derivation),
which gives rise to the NCL update rule
%
\begin{equation}
	\b{\theta} \leftarrow \b{\theta}
	+\gamma
	\left [
		\b{\Lambda}_{k-1}^{-1} \nabla_{\b{\theta}}
		\ell_k(\b{\theta})
		-
		(\b\theta - \b{\mu}_{k-1})
		\right ]
	\label{eq:ncl_update}
\end{equation}
for a learning rate parameter $\gamma$ (which is implicitly a function of $r$ in \Cref{eq:ncl_trust_region}).
%
To get some intuition for this learning rule, we note that $\b{\Lambda}_{k-1}^{-1}$ acts as a preconditioner for the first (likelihood) term, which drives learning on the current task while encouraging parameter changes predominantly in directions that do not interfere with previous tasks.
Meanwhile, the second term encourages $\b{\theta}$ to stay close to $\b{\mu}_{k-1}$, the optimal parameters for the previous task.
As we illustrate in \Cref{fig:schematic}, this combines the desirable features of both Bayesian weight regularization and projection-based methods.
In particular, NCL shares the fixed points of the Bayesian posterior while also mitigating intermediate or complete forgetting of previous tasks by preconditioning with the prior covariance.
Notably, if the loss landscape is non-convex (as it generally will be), NCL can converge to a different local optimum from standard weight regularization despite having the same fixed points (\Cref{fig:schematic}B).


\paragraph{Implementation}
The general NCL framework can be applied with different approximations to the Fisher matrix $\b{F}_k$ in \Cref{eq:fisher_k}~(see \Cref{subsec:bcl}).
In this work, we use a Kronecker-factored approximation \citep{martens2015optimizing,ritter2018online}.
%A major challenge in implementing NCL lies in the computation of $\b{\Lambda}_{k-1}^{-1}$, which is generally intractable for large models.
However, even after making a Kronecker-factored approximation to $\b{F}_k$ for each task $k$, it remains difficult to compute the inverse of a sum of $k$ Kronecker products (c.f.\ \Cref{eq:laplace_update_lambda}).
To address this challenge, we derived an efficient algorithm for making a Kronecker-factored approximation to $\b{\Lambda}_k = \b{F}_k + \b{\Lambda}_{k-1} \approx \b{A}_k \otimes \b{G}_k$ when $\b{\Lambda}_{k-1} = \b{A}_{k-1} \otimes \b{G}_{k-1}$ and $\b{F}_k$ are also Kronecker products.
This approximation minimizes the KL-divergence between $\mathcal{N}(\b{\mu}_k, (\b{A}_k \otimes \b{G}_k)^{-1})$ and $\mathcal{N}(\b{\mu}_k, (\b{\Lambda}_{k-1} + \b{F}_{k})^{-1})$ (see~\CrefNoLink{sec:kron_sums} for details).
Before training on the first task, we assume a spherical Gaussian prior $\b{\theta} \sim \mathcal{N}(\b{0}, p_{w}^{-2} \b{I})$.
The scale parameter $p_w$ can either be set to a fixed value (e.g. 1) or treated as a hyperparameter, and we optimize $p_w$ explicitly for our experiments in feedforward networks.
NCL also has a parameter $\alpha$ which is used to stabilize the matrix inversion $\b{\Lambda}_{k-1}^{-1} \approx (\b{A}_{k-1} \otimes \b{G}_{k-1} + \alpha^2 \b{I})^{-1}$ (\CrefNoLink{sec:implementation}).
This is equivalent to a hyperparameter used for such matrix inversions in OWM \citep{zeng2019continual} and DOWM \citep{duncker2020organizing}, and it is important for good performance with these methods.
The $p_w$ and $\alpha$ are largely redundant for NCL, and we generally prefer to fix $\alpha$ to a small value ($10^{-10}$) and optimize the $p_w$ only.
However, for our experiments in RNNs, we instead fix $p_w=1$ and perform a hyperparameter optimization over $\alpha$ for a more direct comparison with OWM and DOWM.
The NCL algorithm is described in pseudocode in \CrefNoLink{sec:implementation} together with additional implementation and computational details.
Finally, while we have derived NCL with a Laplace approximation in this section for simplicity, it can similarly be applied in the variational continual learning framework of \citet{nguyen2017variational} (\CrefNoLink{sec:vcl}).
Our code is available online\footnote{\href{https://github.com/tachukao/ncl}{https://github.com//tachukao/ncl}}.

\subsection{Related work}
\label{subsec:related}

As discussed in \Cref{subsec:bcl}, our method is derived from prior work that relies on Bayesian inference to perform weight regularization for continual learning \citep{kirkpatrick2017overcoming, nguyen2017variational,huszar2017quadratic,ritter2018online}.
However, we also take inspiration from the literature on natural gradient descent \citep{amari1998natural,kunstner2019limitations} to introduce a preconditioner that encourages parameter updates primarily in flat directions of previously learned tasks (\CrefNoLink{sec:ngd}).

Recent projection-based methods \citep{duncker2020organizing,zeng2019continual,saha2021gradient} have addressed the continual learning problem using an update rule of the form
%
\begin{equation}
	\label{eq:proj_up}
	\b{\theta} \leftarrow \b{\theta} + \gamma \b{P}_L \nabla_{\b{\theta}} \ell_k(\b{\theta}) \b{P}_R,
\end{equation}
%
where $\b{P}_L$ and $\b{P}_R$ are projection matrices constructed from previous tasks which encourage parameter updates that do not interfere with performance on these tasks.
Using Kronecker identities, we can rewrite \Cref{eq:proj_up} as
%
\begin{equation}
	\b{\theta} \leftarrow \b{\theta} + \gamma (\b{P}_R \otimes \b{P}_L) \nabla_{\b{\theta}} \ell_k(\b{\theta}).
\end{equation}
%
This resembles the NCL update rule in \Cref{eq:ncl_update} where we identify $\b{P}_R \otimes \b{P}_L$ with the approximate inverse prior precision matrix used for gradient preconditioning in NCL, $ \b{\Lambda}_{k-1}^{-1}= \b{A}_{k-1}^{-1} \otimes \b{G}_{k-1}^{-1}$.
Indeed, we note that for a Kronecker-structured approximation to $\b{F}_k$, the matrix $\b{A}_{k-1}$ approximates the empirical covariance matrix of the network activations experienced during all tasks up to $k-1$ (\citealp{martens2015optimizing,bernacchia2018exact}, \CrefNoLink{sec:fisher_deriv}), which is exactly the inverse of the projection matrix $\b{P}_R$ used in previous work \citep{duncker2020organizing,zeng2019continual}.
We thus see that NCL takes the form of recent projection-based continual learning algorithms with two notable differences:
\vspace{0.2em}\\
%
(i) NCL uses a \emph{left} projection matrix $\b{P}_L$ designed to approximate the posterior covariance of previous tasks $\b{\Lambda}_{k-1}^{-1} \approx \b{P}_R \otimes \b{P}_L$ (i.e., the prior covariance on task $k$; \CrefNoLink{sec:fisher_deriv}), while \citet{zeng2019continual} use the identity matrix $\b{I}$ and \citet{duncker2020organizing} use the covariance of recurrent inputs (\CrefNoLink{sec:proj}).
Notably, both of these choices of $\b{P}_L$ still provide reasonable approximations to $\b{\Lambda}_{k-1}^{-1}$, and thus the parameter updates of OWM and DOWM can also be viewed as projecting out steep directions of the prior on task $k$ (\CrefNoLink{sec:proj}).
%
\vspace{0.2em}\\
%
(ii) NCL includes an additional regularization term $(\b{\theta} - \b{\mu}_{k-1})$ derived from the Bayesian posterior objective, while \citet{duncker2020organizing} and \citet{zeng2019continual} do not use such regularization.
%
%\vspace{0.2em}\\
%
Importantly, this means that while NCL has a similar preconditioner and optimization path to these projection based methods, NCL has stationary points at the modes of the approximate Bayesian posterior while the stationary points of OWM and DOWM do not incorporate prior information from previous tasks (c.f.\ \Cref{fig:schematic}).

It is also interesting to note that previous Bayesian continual learning algorithms include a hyperparameter $\lambda$ that scales the prior compared to the likelihood term for the current task \citep{loo2020generalized}:
%
\begin{equation}
	\label{eq:L_lambda}
	\mathcal{L}_k^{(\lambda)}( \b{\theta} ) = \log p(\mathcal{D}_k | \b{\theta}) - \lambda (\b{\theta} - \b{\mu}_{k-1})^\top \b{\Lambda}_{k-1} (\b{\theta} - \b{\mu}_{k-1}).
\end{equation}
%
To minimize this loss and thus find a mode of the approximate posterior, it is common to employ pseudo-second-order stochastic gradient-based optimization algorithms such as Adam~\citep{kingma2014adam} that use their own gradient preconditioner based on an approximation to the Hessian of \Cref{eq:L_lambda}.
Interestingly, this Hessian is given by $\b{H}_k = -H(\mathcal{D}_k, \b{\theta}) - \lambda \b{\Lambda}_{k-1}$, which in the limit of large $\lambda$ becomes increasingly similar to preconditioning with the prior precision as in NCL.
Consistent with this, previous work using the online Laplace approximation has found that large values of $\lambda$ are generally required for good performance \citep{kirkpatrick2017overcoming, ritter2018online, van2018generative}.
Recent work has also combined Bayesian continual learning with natural gradient descent \citep{osawa2019practical, tseran2018natural}, and in this case a relatively high value of $\lambda=100$ was similarly found to maximize performance \citep{osawa2019practical}.



==> figures/_fig_kfac_decoupled_lambda.tex <==
\begin{figure}[!t]
    \centering
    \includegraphics[width = 1.\textwidth]{figs/ryang_high_kfac-adam-decoupled_lambda.pdf}
    \caption{\label{fig:kfac_lambda_decoupled}
        %
        {\bfseries Continual learning on SR tasks for different $\lambda$ with decoupled KFAC.}
        {\bfseries (A)}~Log loss for each of the six stimulus-response tasks as a function of optimization step for KFAC with $\lambda = 1$, optimized using decoupled Adam.
        {\bfseries (B-E)}~As in (A), now with values of $\lambda \in [10, 10^2, 10^3, 10^4]$.
        }
    \vspace*{-1em}
\end{figure}



==> figures/_fig_kfac_ryang_lambda.tex <==
\begin{figure}[!t]
    \centering
    \includegraphics[width = 1.\textwidth]{figs/ryang_high_kfac-adam_lambda.pdf}
    \caption{\label{fig:kfac_lambda}
        %
        {\bfseries Continual learning on SR tasks for different $\lambda$ with KFAC.}
        {\bfseries (A)}~Log loss for each of the six stimulus-response tasks as a function of optimization step for KFAC with $\lambda = 1$, optimized using Adam.
        {\bfseries (B-E)}~As in (A), now with values of $\lambda \in [10, 10^2, 10^3, 10^4]$.
        }
    \vspace*{-1em}
\end{figure}



==> figures/_fig_ncl_ryang_lambda.tex <==
\begin{figure}[!t]
    \centering
    \includegraphics[width = 1.\textwidth]{figs/ryang_high_ncl_lambda.pdf}
    \caption{\label{fig:ncl_lambda}
        %
        {\bfseries Continual learning on SR tasks for different $\lambda$ with NCL.}
        {\bfseries (A)}~Log loss for each of the six stimulus-response tasks as a function of optimization step for NCL with $\lambda = 1$.
        {\bfseries (B-E)}~As in (A), now with values of $\lambda \in [10, 10^2, 10^3, 10^4]$.
        }
    \vspace*{-1em}
\end{figure}



==> figures/_fig_ryang_high.tex <==
\begin{figure}[!t]
    \centering
    \includegraphics[width = 1.\textwidth]{figs/ryang_high.pdf}
    \caption{\label{fig:ryang}
        %
        {\bfseries Continual learning on stimulus-response tasks.}
        Evolution of the loss during training for each of the six stimulus-response tasks for NCL (A), DOWM (B), OWM (C), and KFAC with $\lambda = 1$ (D).
        Coloured lines and shadings indicate mean and stdev for each task across 5 random seeds.
        Black lines indicate the mean loss over all tasks at the end of training.
        Task order matches that of \citet{duncker2020organizing}.
        Note that the earlier tasks are also `easier' in a non-continual setting \citep{yang2019task}.
        }
    \vspace*{-1em}
\end{figure}



==> figures/_fig_ryang_low.tex <==
\begin{figure}[!t]
    \centering
    \includegraphics[width = 1.0\textwidth, trim={0 0 0 0}, clip=true]{figs/ryang_low.pdf}
    \caption{\label{fig:ryang_low}
        %
        {\bfseries Continual learning on stimulus-response tasks with a 50-unit RNN.}
        Evolution of the loss during training for each of the six stimulus-response tasks for NCL (A), DOWM (B), OWM (C), and KFAC with $\lambda = 1$ (D).
        Solid black lines indicate the mean loss over all tasks at the end of training.
        }
    \vspace*{-1em}
\end{figure}



==> figures/_fig_smnist.tex <==
\begin{figure}[!t]
    \centering
    \includegraphics[width = 0.80\textwidth, trim={0 0 0 0}, clip=true]{figs/smnist_perf.pdf}
    \caption{\label{fig:smnist}
        %
        {\bfseries Performance on sequential stroke MNIST.}
        {\bfseries (A)}~Classification performance of NGCL, orthogonal and OWM on each task of sequential stroke mnist after training on all tasks.
        Horizontal lines indicate mean across tasks.
        {\bfseries (B)}~Cross-entropy loss on stroke mnist.
        }
    \vspace*{-1em}
\end{figure}


